Uni-NaVid: A Video-based Vision-Language-Action Model for Unifying Embodied Navigation Tasks

A practical navigation agent must be capable of handling a wide range of interaction demands, such as following instructions, searching objects, answering questions, tracking people, and more. Existing models for embodied navigation fall short of serving as practical generalists in the real world, as they are often constrained by specific task configurations or pre-defined maps with discretized waypoints. In this work, we present Uni-NaVid, the first video-based vision-language-action (VLA) model designed to unify diverse embodied navigation tasks and enable seamless navigation for mixed long-horizon tasks in unseen real-world environments. Uni-NaVid achieves this by harmonizing the input and output data configurations for all commonly used embodied navigation tasks and thereby integrating all tasks in one model. For training Uni-NaVid, we collect 3.6 million navigation data samples in total from four essential navigation sub-tasks and foster synergy in learning across them. Extensive experiments on comprehensive navigation benchmarks clearly demonstrate the advantages of unification modeling in Uni-NaVid and show it achieves state-of-the-art performance. Additionally, real-world experiments confirm the model's effectiveness and efficiency, shedding light on its strong generalizability.

==> algo/token_merge_algo_new.tex <==
\begin{algorithm}[t]
\caption{Online Visual Token Merging}
\label{algo:token-merging}
\begin{algorithmic}[1]
\Require 
\Statex
\begin{itemize}
    \item Total number of frames $T$
    \item Short memory buffer length $B$
    \item Grid pooling scales: $\alpha_{\text{curr}}$, $\alpha_{\text{short}}$, $\alpha_{\text{long}}$
    \item Current visual tokens: $\mathbf{X}_T \in \mathbb{R}^{N_x \times C}$
    \item Previously merged tokens: $\mathbf{X}_{\text{curr}}$, $\mathbf{X}_{\text{short}}$, $\mathbf{X}_{\text{long}}$
    \item Number of frames merged in the last tokens of long memory: $K$
\end{itemize}
\Ensure 
\Statex
\begin{itemize}
    \item Updated merged tokens: $\mathbf{X}'_{\text{curr}}$, $\mathbf{X}'_{\text{short}}$, $\mathbf{X}'_{\text{long}}$
    \item Updated number of frames merged in the last tokens of long memory: $K'$
\end{itemize}
\Statex % Blank line for spacing


\State $\mathbf{X}'_\text{curr} \gets GridPool(\mathbf{X}_T, \alpha_\text{curr})$ \Comment{Current visual tokens}


\If{$T > 1$} \Comment{Add short-term visual tokens}
    \State $\mathbf{X}_{\text{curr}\rightarrow\text{short}} \gets GridPool(\mathbf{X}_\text{curr}, \frac{\alpha_{\text{short}}}{\alpha_{\text{curr}}})$
    \State $\mathbf{X}'_{\text{short}} \gets \mathbf{X}_{\text{short}} + [\mathbf{X}_{\text{curr}\rightarrow\text{short}}]$
    
    \If{$T>B+1$} \Comment{Add long term visual tokens}
        \State $\mathbf{X}_{\text{short}\rightarrow\text{long}} \gets GridPool(\mathbf{X}_\text{short}[0], \frac{\alpha_{\text{long}}}{\alpha_{\text{short}}})$
        \State $\mathbf{X}'_{\text{short}} \gets \mathbf{X}_{\text{short}}[1:]$
        \State $s \gets \cos(\mathbf{X}_{\text{long}}[-1], \mathbf{X}_{\text{short}\rightarrow\text{long}})$

    
    \EndIf
    % \State return
% \Else
%     \State $\mathbf{X}_{\text{curr}\rightarrow\text{short}} \gets GridPool(\mathbf{X}_\text{curr}, \frac{\alpha_{\text{short}}}{\alpha_{\text{curr}}})$
%     \State $\mathbf{X}'_{\text{short}} \gets \mathbf{X}_{\text{short}} + [\mathbf{X}_{\text{curr}\rightarrow\text{short}}]$
\EndIf




\If{$T > B+1$}
    \State $\mathbf{X}_{\text{short}\rightarrow\text{long}} \gets GridPool(\mathbf{X}_\text{short}[0], \frac{\alpha_{\text{long}}}{\alpha_{\text{short}}})$
    \State $\mathbf{X}'_{\text{short}} \gets \mathbf{X}_{\text{short}}[1:]$
    %\State $\text{m}\gets $
    \State $s \gets \cos(\mathbf{X}_{\text{long}}[-1], \mathbf{X}_{\text{short}\rightarrow\text{long}})$
    \If{$T>B+2\ \text{and}\ s>\tau$}
        \State $\mathbf{X}_{\text{last\_long}} \gets \frac{1}{K+1}(K\mathbf{X}_{\text{long}}[-1]+\mathbf{X}_{\text{short}\rightarrow\text{long}})$
        \State $\mathbf{X}'_{\text{long}} \gets \mathbf{X}_{\text{long}}[:-1] + [\mathbf{X}_{\text{last\_long}}]$
        \State $K'\gets K+1$
    \Else
        \State $\mathbf{X}'_{\text{long}} \gets \mathbf{X}_{\text{long}} + [\mathbf{X}_{\text{short}\rightarrow\text{long}}]$
        \State $K'\gets 1$
    \EndIf
\EndIf


\end{algorithmic}
\end{algorithm}

==> fig/data_synergy.tex <==
\begin{figure}[t]
\begin{center}
  \includegraphics[width=1\linewidth]{fig/img/data_plot.pdf}
\end{center}
   \caption{\textbf{Ablation study of traing strategy.}}
\label{fig:data}
% \vspace{-5mm}
\end{figure}




==> fig/teaser.tex <==
\begin{figure*}[t]
\begin{center}
  \includegraphics[width=1 \linewidth]{fig/img/teaser.pdf}
\end{center}
   \caption{\name~learns general navigation skills across four embodied navigation tasks using 3.6 million navigation samples. \name~only takes online RGB video frames and language instructions as input and output actions, achieving general navigation ability in a real-world deployment. }
\label{fig:teaser}
% \vspace{-5mm}
\end{figure*}




==> fig/time_analyze.tex <==
\begin{figure}[t]
\begin{center}
  \includegraphics[width=1 \linewidth]{fig/img/time_analyze.pdf}
\end{center}
   \caption{\textbf{Time efficiency visualization.} We provide the average
running time and the number of tokens across different time steps.}
\label{fig:time_analyze}
% \vspace{-5mm}
\end{figure}




==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

% \input{fig/teaser}

% Embodied navigation is fundamental for supporting various interaction demands. Recently, instruction-following navigation techniques have advanced significantly with the development of multimodal models. However, existing studies~\cite{anderson2018evaluation, wu2024embodied, zheng2023towards, long2024instructnav, zhou2023navgpt, shah2023gnm, Zhang2024VisionandLanguageNT,shah2023navigation, robinson2023robotic,zhang20233d} either develop individual models for different tasks, \egno, vision-and-language navigation~\cite{Krantz2020BeyondTN, anderson2020rxr}, object goal navigation~\cite{chaplot2020object}, embodied question answering~\cite{das2018embodied}, following~\cite{zhang2021efficient, huang2017robust, puig2023habitat}, \etcno, or explore task unification in a simplified setting (Tab.~\ref{tab:comp-task}). They all fall short as full-stack navigation models qualified for practical general-purpose deployment.
% in the real world.
% and have not make full use of the available datasets.

Navigation is a critical capability for intelligent robots drawing considerable attention from both computer vision~\addcite and robotics~\addcite fields. For successful navigation, robots must be able to move autonomously within physical environments according to human instructions. However, navigation tasks vary significantly, each demanding unique skills based on the type of instructions, such as object-goal navigation, vision-and-language navigation, and more. Consequently, most current approaches are developed to address only one type of navigation task, often relying on specialized modules and task-specific datasets. This narrow scope limits their utility to single-purpose applications, preventing these models from leveraging potential synergies across diverse navigation tasks.

% Such as object goal navigation task~\addcite~ requires the robot to explore the environment and identify the target objects. While vision-and-language Navigation~\addcite~ requires the robot to follow the motion to approach recognized landmarks step by step. 
% Instead, humans have an innate ability to easily interpret scenes and complete various navigation tasks, a skill that naturally supports general navigation ~\addcite.

However, building the general navigation model for intelligent robots is particularly challenging because it requires the model to master different navigation capabilities in one single framework with unified observation encoding and action prediction strategies. Early attempts using imitation learning (IL)~\addcite or reinforcement learning (RL)~\addcite directly learn general navigation capability from synthetic environments. However, these works suffer from the sim-to-real gap, leading to poor generalist performance when transferred to novel environments, including novel datasets and real worlds.



% Developing a full-stack navigation model poses significant challenges, not only in unifying task modeling but also in integrating heterogeneous data in joint use. Initial efforts adopt imitation learning (IL)~\cite{wang2022towards,wu2020towards, nguyen2019vision} or reinforcement learning (RL)~\cite{zeng2024poliformer, xu2023benchmarking} to learn general navigation skills in simulation environments or limited diverse real-world environments. 
% These methods have shown promise in synthetic environments. 
% However, due to the limited rendering quality and diversity of simulators, these approaches often encounter the ``sim-to-real'' gap and suffer from poor generalization across diverse navigation tasks~\cite{gervet2023navigating, anderson2021sim, kadian2020sim2real}. Recent studies~\cite{zhou2023navgpt, zheng2023towards, long2024instructnav, long2023discuss,shah2023lm} have attempted to achieve a higher degree of unification on top of pre-trained LLMs, but they simplify the problem to some extent by adopting discretized modeling approaches. They rely on pre-defined graphs for learning decision-making, thus sacrificing the output flexibility and resulting in a low upper bound, especially for real-world deployment. 

Developing a general navigation model for intelligent robots poses significant challenges, as it demands a unified framework while requiring data or modules that support general navigation tasks. Initial efforts using imitation learning (IL)\addcite or reinforcement learning (RL)\addcite aimed to learn general navigation skills within synthetic environments on simulators. These methods have shown promise in synthetic environments. However, due to the limited rendering quality and diversity of simulators, these approaches often encounter the ``sim-to-real'' gap and poor generalization across diverse navigation tasks.


Recent advancements in large language models (LLMs) have demonstrated remarkable open-world generalization capabilities, inspiring new approaches that leverage LLMs for creating general navigation agents. However, adapting LLMs to computationally intensive navigation tasks remains challenging. Some methods utilize pre-trained LLMs (e.g., ChatGPT~\cite{OpenAI2023ChatGPT}, Llama~\cite{touvron2023llama}) with text prompts to describe scenes, while others rely on end-to-end training using images of discrete landmarks. These approaches signal the dawn of general navigation, yet the reliance on text prompts and landmark images limits environmental awareness, hindering performance and complicating real-world deployment. This raises the question: \textit{can we train a large model that incorporates compact and dense observations, supports diverse instructions, and maintains high efficiency for practical deployment?}

Recently, large language models have exhibited impressive open-world generalization capacities which inspired advanced works that leverage large language models for building general navigation agents. To use LLM run computational dense navigation task, these types of works either use off-the-shelf LLM (ChatGPT~\addcite, LLama~\addcite) with text prompts for scene description or end-to-end training using images of discrete landmarks. Both strategies lead to insufficient observation of the environment, leading to performance damage and making real-world deployment inconvenient.  

% The question is: \textit{can we directly train a large model for navigation that supports general instructions and is able to run efficiently?}

% In this paper, we lean toward another perspective and ask the following question: Toward a reliable and planning-oriented autonomous driving system, how to design the pipeline in favor of planning? which preceding tasks are requisite?



% The question is: \textit{can we directly train a large model for navigation that supports general instructions and is able to run efficiently?}

% can not provide detailed information for online navigation, or for conveniently real-world deployment.



% One widely used way is to leverage the text prompt to describe the scene environment and instructions and use 



% (LLM)~\addcite, \addcite~ leverages the text prompt to describe the scene environment and instructions for selecting discrete landmarks. However, the text prompts could suffer severe information drop when distilled from visual information, and the inference frequency makes these methods unable to run at online manner. The question is: \textit{can we directly train a large model for navigation that supports general instructions and is able to run efficiently?}


% In this work, we propose \name, a Vision-Language-Action (VLA) model for unifying diverse commonly demanded navigation tasks (Tab.~\ref{tab:comp-task}). It takes video streams and natural language as input, adaptively generates actions following instructions, and automatically responds to questions if raised in an end-to-end manner. We make the first endeavor to address three essential questions, as elaborated below, in pursuit of ultimate real-world application.

% \textit{How to unify different navigation tasks with minimal problem simplification and maximum utilization of data?} We target an up-to-date unification modeling in \name{} where it takes single-view egocentric video streams and natural language as inputs, and end-to-end generate actions or linguistic responses for instructions or questions adaptively. We follow the natural characteristic of Large Language Models (LLMs) to cross-modally interleave the inputs and outputs of different navigation tasks into a single sequence in the token space to enable joint learning with \textit{next-token-prediction} paradigm for \name. It incorporates four widely demanded navigation tasks, including Vision-and-Language Navigation (VLN), object-goal navigation, embodied question answering, and human following. The corresponding training data are all collected from simulation environments. Besides, we further incorporate Internet real-world data for Video Question Answering (VQA)~\cite{azuma2022scanqa,li2023llama} and video captioning~\cite{chen2024panda} as auxiliary tasks into this unified model to enhance navigation performance and promote sim-to-real generalization. This is a groundbreaking attempt in this field at unified cross-modal, cross-task, and cross-sim-to-real modeling. It achieves impressive synergy in a broad range and results in a full-stack navigation agent.

% \textit{How to improve the efficiency of such a unification design to enable a deployment-friendly model?} In addition to unification modeling, we also prioritize efficient model design for practical deployment. Specifically, we adopt an online token merging mechanism to compress near historical frames with a relatively low ratio while compressing far historical frames with a relatively high ratio. In this way, \name{} learn compact representations that maintain not only fine-grained spatial information but also structured temporal information, thus speeding up the model inference by reducing the token number. Besides, \name~adopts a foresight prediction to generate actions for a future horizon at once instead of step-by-step. This allows us to use an asynchronous strategy for action inference and execution.

% \textit{How to verify the synergy between different tasks?} We conduct comprehensive ablation studies to verify the synergy over different navigation tasks, as well as between simulation and real-world tasks in both simulation and real-world environments. We find they promote each other with unification modeling in such a broad range and help \name{} attain clear superiority in all sub-tasks~\cite{Krantz2020BeyondTN,savva2019habitat,das2018embodied,islam2019person} compared to recent works. Besides, we also evaluate \name{} on long-horizon real-world tasks, which include multiple subtasks, and witness it can complete them in a zero-shot manner as shown in Figure~\ref{fig:teaser}. 

% By exploring these three essential questions, we demonstrate the advantages of unified modeling and joint data utilization across different tasks and in sim-to-real transfer. We hope this will foster future progress in developing an up-to-date full-stack navigation agent for general-purpose real-world applications.
% We witness it achieves impressive synergy in a broad range and results in a full-stack navigation agent capable of zero-shot completing long-horizon real-world tasks, which includes multiple subtasks, as shown in our teaser figure.

% ============ Version 1.0 (Re-organized) ===========================

We introduce \name{}, an end-to-end video-based large language model for general navigation tasks. \name{} serves as a unified framework, using natural language as instructional input and streaming video as visual input to support diverse navigation tasks.
% such as object-goal navigation, vision-and-language navigation, human following, and embodied question answering.
Built on a vision-language model~\cite{vicuna2023}, \name{} benefits from open-world knowledge and robust generalization capabilities to comprehend novel text and instructions. 
Unlike the more widely studied image or video question-answering tasks~\addcite, navigation requires processing large volumes of continuous video frames, which often leads to memory overload and inefficiencies. To address this, we employ a memory fusion technique that consolidates visual information both spatially and temporally.
Specifically, we online organize video frames into instant observation, short-term memory, and long-term memory, and encode these frames to visual tokens. With the rule that the latest information is more important for navigation, we gradually fuse visual tokens for each type of memory.
This design leads five times faster than naive video-based vision-language models~\addcite with better navigation performance. 



% % \name{}~ adopts the Atkinson–Shiffrin memory model\addcite, which organizes the video temporal information into instant memory, short-term memory, and long-term memory. With the rule that the latest information is more important for navigation, we adaptive fuse temporal information for each type of memory, allowing \name{}~ to operate five times faster than naive video-based vision-language models with better navigation performance. 



We trained \name{} on a large, self-collected navigation dataset containing 3.6 million video-action samples spanning four navigation tasks (see Figure~\ref{fig:teaser}). These navigation samples are collected from existing datasets in a unified format, including an egocentric video, natural language instructions, and the corresponding next actions. Although we aimed to gather a wide variety of samples, the diversity of environments within existing datasets limits the breadth of our navigation data, making it challenging to achieve truly open-vocabulary data coverage. 
To address this, inspired by the success of VLA models~\addcite, we co-tuned \name{} with open-world data from text, image, and video QA tasks, treating them as different modalities of our model. 
This training strategy led to substantial improvements in generalization across objects, scenes, and instructions, and enabled zero-shot navigation capabilities in real-world environments.


% % We try our considerable effort to collect as diverse samples as possible, however, limited to the diversity of environments of each dataset, it's impossible to achieve open-vocabulary level navigation data. Inspired by the success of VLA models~\addcite, we co-tuning our model open-world text, image and video QA data, by formulating them as different modalities of observations of \name{}. We find that this training strategy enables significant improvements to generalization over objects, scenes, and instructions, and exhibits zero-shot performance on real-world environment.



% % To make the training more efficient, we use a curriculum learning strategy ~\addcite to learn basic navigation skills and then learn advanced navigation skills that involve free-form linguistic instructions and diverse environments.  
% %
% % Firstly, \name{}~ was trained with 500K simple basic navigation video-action samples, such as moving forward or turning right a few steps, or combinations of these basic movements. After mastering the basic navigation skills, \name{}~ was trained with 3.1 million navigation video-action samples across various navigation tasks, including vision-and-language navigation, object goal navigation, human following and embodied question answering. \todo{Add real-world data descriptions.}


We conduct extensive experiments on both synthetic and real-world environments, Extensive experiments on both simulated and real-world environments demonstrate that \name{} archives SOTA-level performance across different navigation tasks and strong generalization capabilities beyond the training dataset. \name{} improves the VLN-CE RxR benchmark from $36\%$ to $52\%$\td{check the number} and achieves SOTA zero-shot object goal navigation performance using only a limited set of object categories during training.


==> table/human_following_mp3d.tex <==
\begin{table}[!t]
\centering

% \vspace{-5pt}
% \resizebox{\linewidth}{!}{
\scalebox{0.8}{
\setlength{\tabcolsep}{0.8mm}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{l|cc|ccc}
\hline
\multirow{2}{*}{Method} & \multicolumn{2}{c|}{Observation} & \multicolumn{3}{c}{HF-MP3D} \\
& H.Det. & S.RGB & \hspace{0.3cm}\textbf{SR}$\uparrow$\hspace{0.2cm} & \hspace{0.2cm}\textbf{FR}$\uparrow$\hspace{0.2cm} & \hspace{0.2cm}\textbf{CR}$\downarrow$ \\
\hline

PoliFormer~\cite{zeng2024poliformer}     &  & $\checkmark$ & 2.62 & 16.59 & 1.43 \\
PoliFormer$^*$~\cite{zeng2024poliformer}     & $\checkmark$ & $\checkmark$ & 25.42 & 47.80 & 8.72 \\
PoliFormer$\dag $~\cite{zeng2024poliformer}     & $\checkmark$ & $\checkmark$ & 21.90 & 41.42 & 7.15 \\
IBVS$^*$~\cite{gupta2016novel} & $\checkmark$ & $\checkmark$ & 56.86 & 68.91 & 1.33 \\
IBVS$\dag $~\cite{gupta2016novel} & $\checkmark$ & $\checkmark$ & 58.15 & 65.83 & \textbf{0.77} \\
\textbf{\name}           & & $\checkmark$ & \textbf{69.80} & \textbf{78.96} & 2.99 \\ \hline
\end{tabular}
}
}
\caption{\textbf{Human following.} Comparison on Human Following MP3D Benchmark (HF-MP3D). $^*$: Methods use GroundingDINO~\cite{liu2023grounding} as the open-vocabulary human detector. $\dag$: Methods use the ground-truth bounding box provided by the simulator.}
\label{tab:human-following}
\vspace{-3mm}
\end{table} 


